Benchmarks for single-phase flow in fractured porous media

This paper presents several test cases intended to be benchmarks for numerical schemes for single-phase fluid flow in fractured porous media. A number of solution strategies are compared, including a vertex and a cell-centered finite volume method, a non-conforming embedded discrete fracture model, a primal and a dual extended finite element formulation, and a mortar discrete fracture model. The proposed benchmarks test the schemes by increasing the difficulties in terms of network geometry, e.g. intersecting fractures, and physical parameters, e.g. low and high fracture-matrix permeability ratio as well as heterogeneous fracture permeabilities. For each problem, the results presented by the participants are the number of unknowns, the approximation errors in the porous matrix and in the fractures with respect to a reference solution, and the sparsity and condition number of the discretized linear system. All data and meshes used in this study are publicly available for further comparisons.

==> introduction.tex <==
Many fields of applications for porous media flow include geometrically
anisotropic inclusions and strongly discontinuous material coefficients which
differ in orders of magnitude. If the extension of those heterogeneities is
small in normal direction compared to the tangential directions,
those features are called fractures. Examples which include such fractured
porous-media systems in earth sciences include reservoir engineering,
groundwater-resource management, renewable energy storage, oil and gas
recovery, radioactive-waste reposition, coal bed methane migration in mines,
geothermal engineering and hydraulic fracturing.

The analysis and prediction of flow in fractured porous-media systems is
important for all the aforementioned applications. Many different conceptual and
numerical models of flow in fractured porous-media systems can be found in the
literature. Even though fractured porous-media systems have been of interest to
modelers for a long time, they still represent challenges for simulators.
However, even in the time of large supercomputers with massive parallel
computing power, the computational efficiency, and implicitly the economic
efficiency, plays an important role in the evaluation of simulation software.

During the last 70 years, different modeling approaches have been developed and
gradually improved. Comprehensive reviews can be found in
\cite{berkowitz2002characterizing,dietrich2005flow,hoteit2008numerical,neumann2005review,sahimi2011flow,singhal2010applied}.
Roughly, the fractured porous media systems are classified in two broad
categories: discrete fracture matrix  (DFM) models and continuum fracture
models. Within this paper, we will only consider DFM models.

The DFM models consider flow occurring both in the fracture network and the
surrounding rock matrix. They account explicitly for the effects of individual
fractures on the fluid flow. An efficient way to represent the fractures in DFMs
is the hybrid-dimensional approach, e.g.
\cite{helmig_multiphase_1997,firoozabadi_control-volume_2004,reichenberger_mixed-dimensional_2006},
where fractures are discretized with elements of co-dimension one with respect
to the surrounding matrix such as one-dimensional elements in two-dimensional
settings. The aforementioned classical DFM approaches all rely on matching fracture and
matrix grids in the sense that a fracture element is geometrically coincinding
with co-dimension-one entities, i.e. faces, of matrix grid elements.
In addition to those, several so-called non-conforming DFM models have been developed
in recent years, such as EDFM \cite{}, XFEM-based approaches
\cite{dangelo2012mixed,Schwenck:2015:DRF}, or mortar-type methods \cite{}.

The main focus of this work is to reuse existing and propose new
computational benchmarks for fluid flow in fractured porous media in order to
compare several DFM models.
We would also like to invite the scientific community to follow up on our
study and evaluate further methods by means of the proposed benchmarks.
In order to facilitate this, the paper is accompanyied by grid and result
files in form of a Git repository.

The remainder of this paper is organized as follows.
In Section \ref{sec:model}, we formulate the model problem in terms of
the partial differential equation that is to be solved.
The participating DFM models are described in Section \ref{sec:methods}.
The central Section \ref{sec:benchmarks} proposes the benchmarks and
compares the results of those methods.
Finally, Section \ref{sec:summary} concludes with a summary and outlook.

